Learning to Rank Normalized Entropy Curves with Differentiable Window Transformation

Recent automated machine learning systems often use learning curves ranking models to inform decisions about when to stop unpromising trials and identify better model configurations. In this paper, we present a novel learning curve ranking model specifically tailored for ranking normalized entropy (NE) learning curves, which are commonly used in online advertising and recommendation systems. Our proposed model, self-Adaptive Curve Transformation augmented Relative curve Ranking (ACTR2), features an adaptive curve transformation layer that transforms raw lifetime NE curves into composite window NE curves with the window sizes adaptively optimized based on both the position on the learning curve and the curve's dynamics. We also introduce a novel differentiable indexing method for the proposed adaptive curve transformation, which allows gradients with respect to the discrete indices to flow freely through the curve transformation layer, enabling the learned window sizes to be updated flexibly during training. Additionally, we propose a pairwise curve ranking architecture that directly models the difference between the two learning curves and is better at capturing subtle changes in relative performance that may not be evident when modeling each curve individually as the existing approaches did. Our extensive experiments on a real-world NE curve dataset demonstrate the effectiveness of each key component of ACTR2 and its improved performance over the state-of-the-art.

==> curve_ranker/dataset.tex <==
\section{Dataset}

==> curve_ranker/related_work.tex <==
\section{Related Work}

Most of the prior work related to learning curve ranking has focused on the pointwise prediction of final individual model performance using partial learning curves. Some approaches, such as~\cite{jamieson2016non,li2017hyperband}, simply used the last observed point on the learning curve to determine when to stop unpromising trials. Others, such as~\cite{mohr2021towards,mohr2021fast}, extrapolated the curve based on the slope of the last two observed points and used a fixed threshold to make termination decisions. Another line of approaches, such as~\cite{domhan2015speeding,chandrashekaran2017speeding,klein2016learning}, used an ensemble of parametric formulas to estimate performance based on partial learning curves, with the parameters calibrated to fit the observed curves. 
Without relying on those basic formulas, the work in \cite{baker2017accelerating} proposed to directly forecast the final performance based on extracted features of the observed curves using a regressive model. All these pointwise approaches rely on curve extrapolation to determine relative superiority and tend to introduce more errors during the extra step. In addition, pointwise ranking has been proven to be less efficient than pairwise ranking that directly optimize for relative superiority~\cite{burges2005learning}. 
Recently work in~\cite{wistuba2020learning} was the first to formulate learning curve ranking as a pairwise ranking problem, and its underline model has achieved state-of-the-art performance in ranking partial learning curves from models across domains. However, the Siamese ranking structure used in~\cite{wistuba2020learning} is not well-suited for ranking curves with small differences, especially when those differences are inconsistent throughout the training process.

In contrast to these previous approaches, our work focuses on directly modeling the difference between learning curves in order to accurately capture subtle patterns of relative change. While building upon pairwise ranking, our proposed framework is specifically tailored for the unique characteristics of NE curves, which are widely used in the computing industry. This makes our work complementary to the previous approaches, and our proposed adaptive curve transformation scheme can be used in conjunction with these methods.

% In parallel to our effort in 
